Soft Constraints for Quality Aspects in Service Oriented Architectures

We propose the use of Soft Constraints as a natural way to model Service Oriented Architecture. In the framework, constraints are used to model components and connectors and constraint aggregation is used to represent their interactions. The "quality of a service" is measured and considered when performing queries to service providers. Some examples consist in the levels of cost, performance and availability required by clients. In our framework, the QoS scores are represented by the softness level of the constraint and the measure of complex (web) services is computed by combining the levels of the components.

==> eptcsdata.tex <==
\providecommand{\event}{M.H. ter Beek (Ed.): Young Researchers Workshop\\
on Service-Oriented Computing 2009 (YR-SOC'09).
}
\providecommand{\volume}{2}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{51}
\providecommand{\eid}{5}

